Checking Causal Consistency of Distributed Databases

The CAP Theorem shows that (strong) Consistency, Availability, and Partition tolerance are impossible to be ensured together. Causal consistency is one of the weak consistency models that can be implemented to ensure availability and partition tolerance in distributed systems. In this work, we propose a tool to check automatically the conformance of distributed/concurrent systems executions to causal consistency models. Our approach consists in reducing the problem of checking if an execution is causally consistent to solving Datalog queries. The reduction is based on complete characterizations of the executions violating causal consistency in terms of the existence of cycles in suitably defined relations between the operations occurring in these executions. We have implemented the reduction in a testing tool for distributed databases, and carried out several experiments on real case studies, showing the efficiency of the suggested approach.

==> summary-of-differences.tex <==
\section{Summary of Differences}
This paper is an extended version of our paper published in NETYS'2019 proceeding\cite{DBLP:conf/NETYS/ZennouBBEE2019}. Since the experiment results have shown that the \texttt{CM} verification cost grows much faster than \texttt{CC} and \texttt{CCv} verification, we extend this work by proposing an optimized definition of the causal memory model \texttt{CM}. The idea is that instead of computing the happen-before relation for all operations as it was defined in \cite{DBLP:conf/popl/BouajjaniEGH17}, we have proved that it is enough to compute it for a small subset of operations to decide for all operations. The experimental results show that this new definition leads to better conformance checking procedure and reduce the \texttt{CM} verification cost by more than 7 times (for histories with 600 operations).
